Operating an Agent-Driven Dataset Factory: Discovery, Construction, and Public Release

Turning public data into prediction datasets requires connecting source discovery, task definition, construction, and distribution. We deployed Dataset Factory to perform these steps continuously under a standing release policy. Bounded language-model tasks interpret sources, write construction code, and review task meaning; deterministic software manages state, workers, retries, and publication. Over 81.53 hours, the factory published 14 datasets at an estimated recurring operating expenditure of about \$2.74 per publication. The accounting includes failed attempts, inference, workers, and hosting. Separate agents completed prediction experiments on all twelve evaluated releases. Source review nevertheless identified a task whose construction filters contradicted its population declaration. The original reviewer accepted later-record exclusions without reconciling them with the published selection rule. This experience documents an operating source-to-release workflow and shows why successful execution and consumer use need separate checks of task meaning.

==> generated/attempt-rows.tex <==
Discover & 54 & 101 & 0 & 30 & 0 & 0 & 185\\
Build & 37 & 260 & 0 & 1 & 0 & 1 & 299\\
Evaluate & 14 & 4 & 21 & 0 & 2 & 0 & 41\\
Publish & 14 & 1 & 0 & 0 & 0 & 0 & 15\\
\midrule
Total & 119 & 366 & 21 & 31 & 2 & 1 & 540\\


==> generated/release-rows.tex <==
Trial within 36 months (courts) & Condition: post-filing jury information; retrospective use. & Stated \\
Reliability deterioration (electricity) & Condition: lagged outcomes require restricted scoring access. & Access stated \\
Penalty reduction (pipelines) & Concern: original-notice timing is unverified. & Partly stated \\
Five-year recall (medical devices) & Concern: undated recalls can become negatives; incidence unverified. & Not found \\
Route survival (aviation) & Condition: carrier-code changes can count as entries or exits. & Exits stated; entries not found \\
Phase I to II award (research grants) & Contradiction: selection declaration; concern: award-amount timing. & Selection: conflicting statements; timing: partly stated \\
Violation escalation (air regulation) & Concern: episode-resolution rule; incidence unverified. & Not found \\
Wastewater exceedance (wastewater) & Condition: prior-year outcome requires restricted scoring access. & Access stated \\
Strike damage (aviation) & Condition: retrospective reports with known damage outcomes. & Stated \\
Permit completion (construction) & Concern: post-issuance field updates are unverified. & Stated \\
Hazmat release (railways) & Condition: retrospective accident-report fields. & Stated \\
Next-period lead exceedance (water) & Concerns: older-history overlap, unit magnitudes, embargo selection. & Overlap and units: not found; embargo: partly stated \\
Record survival (streamgages) & Not evaluated. & Not evaluated \\
Advisory duration (beaches) & Not evaluated. & Not evaluated \\

